Efficient Postprocessing Procedure for Evaluating Hamiltonian Expectation Values in Variational Quantum Eigensolver

We proposed a simple strategy to improve the postprocessing overhead of evaluating Hamiltonian expectation values in Variational quantum eigensolvers (VQEs). Observing the fact that for a mutually commuting observable group G in a given Hamiltonian, <b|G|b> is fixed for a measurement outcome bit string $b$ in the corresponding basis, we create a measurement memory (MM) dictionary for every commuting operator group G in a Hamiltonian. Once a measurement outcome bit string $b$ appears, we store $b$ and <b|G|b> as key and value, and the next time the same bit string appears, we can find <b|G|b> from the memory, rather than evaluate it once again. We further analyze the complexity of MM and compare it with commonly employed post-processing procedure, finding that MM is always more efficient in terms of time complexity. We implement this procedure on the task of minimizing a fully connected Ising Hamiltonians up to 20 qubits, and $H_2$, $H_4$, $LiH$, and $H_2O$ molecular Hamiltonians with different grouping methods. For Ising Hamiltonian, where all $O(N^2)$ terms commute, our method offers an $O(N^2)$ speedup in terms of the percentage of time saved. In the case of molecular Hamiltonians, we achieved over $O(N)$ percentage time saved, depending on the grouping method.

==> table/indicators.tex <==
\begin{table}
\begin{center}
\begin{tabularx}{0.47\textwidth} { 
  | >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X
   >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X | } 
  \hline
  DOW & WILL5000INDFC & VIXCLS\\

  T10Y2Y & T10YIE & DCOILBRENTEU\\
  
  DEXCHUS & DFF & EXPTOTUS \\

  IGREA &  &\\
  \hline
\end{tabularx}
\caption{Financial indicators used as feature for predicting investor's views. Downloaded form Federal Reserve Bank of St. Louis \cite{fred1997}.}
\label{table:indicators}
\end{center}
\end{table}


==> table/opt.tex <==
\begin{table*}[h!]

\begin{subtable}{\textwidth}
\centering
\begin{tabular}{ |c|c|c| }
\hline
Time segment & VQE AR & QAOA AR\\
\hline
1 & 0.979 & 0.721 \\
\hline
2 & 1.0 & 0.715 \\
\hline
3 & 0.914 & 0.612 \\
\hline
4 & 0.911 & 0.83 \\
\hline
5 & 0.992 & 0.892 \\
\hline
6 & 0.965 & 0.919 \\
\hline
7 & 0.97 & 0.871 \\
\hline
8 & 0.983 & 0.512 \\
\hline
9 & 1.0 & 0.923 \\
\hline
\end{tabular}
\caption{Case 1 (individual stocks) optimization results for VQE, QAOA and exhaustive search.}
\label{table:opt1}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\begin{tabular}{ |c|c|c|c|c|c|c|c|c| }
\hline
     Time segment     &  Train & Test & VQE & AR & QAOA & AR & Exact \\
\hline
   1 & 2007-12-31 $\sim$ 2012-12-17&  2012-12-24 $\sim$ 2013-12-16 & 1011101000110001 &0.97 &  &  &1111100011100000\\
\hline
   2 & 2008-12-29 $\sim$ 2013-12-16&  2013-12-23 $\sim$ 2014-12-25 & 0101011010010011 &1.0 &  &  &0001011011110001\\
\hline
   3 & 2009-12-28 $\sim$ 2014-12-15&  2014-12-22 $\sim$ 2015-12-14 & 0111001011100100 &0.96 &  &  &0000001011110111\\ 
\hline
   4 & 2010-12-27 $\sim$ 2015-12-14&  2015-12-21 $\sim$ 2016-12-12 & 0111000011100110 &0.96 &  &  & 0110001011110100\\
\hline
   5 & 2011-12-26 $\sim$ 2016-12-12&  2016-12-19 $\sim$ 2017-12-11 & 1011100010101100 &0.96 &  &  &1111110000110000\\
\hline   
   6 & 2012-12-24 $\sim$ 2017-12-11&  2017-12-18 $\sim$ 2018-12-10 & 1011100011110000 &0.93 &  &  & 1111111000100000\\
\hline   
   7 & 2013-12-23 $\sim$ 2018-12-10&  2018-12-17 $\sim$ 2019-12-09 & 1010111000110001 &0.97 &  &  & 1011101010100010\\
\hline   
   8 & 2014-12-22 $\sim$ 2019-12-09&  2019-12-16 $\sim$ 2020-12-07 & 1010101000110011 &0.92 &  &  & 1000100110110011\\
\hline   
   9 & 2015-12-21 $\sim$ 2020-12-07&  2020-12-14 $\sim$ 2021-12-06 & 1010101010110001 &0.94 &  &  & 1000101011010101\\
\hline
\end{tabular}
\caption{Case 2 (global assets) optimization results for VQE, QAOA and exhaustive search.}
\label{table:opt2}
\end{subtable}

\caption{Optimization solutions.}
\end{table*}

==> table/qml_score1.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ |c|c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| } 
    \hline
    & \multicolumn{2}{c|}{IPG} & \multicolumn{2}{c|}{HAS}  & \multicolumn{2}{c|}{MAR} & \multicolumn{2}{c|}{VLO} & \multicolumn{2}{c|}{GL} & \multicolumn{2}{c|}{MDT} & \multicolumn{2}{c|}{MMM} & \multicolumn{2}{c|}{HPQ} & \multicolumn{2}{c|}{ADSK} & \multicolumn{2}{c|}{NUE} &  \multicolumn{2}{c|}{PLD} & \multicolumn{2}{c|}{XEL} & \multicolumn{2}{c|}{mean} \\
    %\multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c|}{$\qquad$} \\
    \hline
    & $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$ \\
   
    \hline
QSVM & 0.92 & 0.9 & 0.98 & 0.88 & 0.97 & 0.88 & 0.92 & 0.84 & 0.96 & 0.93 & 0.92 & 0.94 & 0.93 & 0.91 & 0.9 & 0.85 & 0.9 & 0.91 & 0.89 & 0.95 & 0.91 & 0.92 & 0.98 & 0.83 & 0.93  &  0.9 \\
\hline
QNN & 0.76 & 0.75 & 0.83 & 0.72 & 0.78 & 0.75 & 0.75 & 0.75 & 0.79 & 0.76 & 0.74 & 0.78 & 0.82 & 0.78 & 0.77 & 0.72 & 0.78 & 0.77 & 0.73 & 0.72 & 0.77 & 0.78 & 0.82 & 0.65 & 0.78  &  0.74 \\
\hline
SVM & 0.92 & 0.91 & 0.97 & 0.88 & 0.95 & 0.91 & 0.93 & 0.83 & 0.94 & 0.93 & 0.9 & 0.92 & 0.92 & 0.9 & 0.93 & 0.81 & 0.9 & 0.9 & 0.85 & 0.92 & 0.93 & 0.88 & 0.98 & 0.83 & 0.93  &  0.89 \\
\hline
NN & 0.86 & 0.87 & 0.93 & 0.76 & 0.95 & 0.82 & 0.86 & 0.75 & 0.96 & 0.86 & 0.86 & 0.87 & 0.93 & 0.86 & 0.91 & 0.74 & 0.86 & 0.86 & 0.85 & 0.93 & 0.91 & 0.83 & 0.98 & 0.71 & 0.91  &  0.82 \\
\hline
  
\end{tabular}}
\caption{Testing accuracy of 4 ML models for each assets. Each score is the average of all 9 time segments.}
\label{table:qml_score1}
\end{table*}


==> table/qml_scores.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{table*}[t]
\begin{subtable}{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ |c|c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| } 
    \hline
    & \multicolumn{2}{c|}{IPG} & \multicolumn{2}{c|}{HAS}  & \multicolumn{2}{c|}{MAR} & \multicolumn{2}{c|}{VLO} & \multicolumn{2}{c|}{GL} & \multicolumn{2}{c|}{MDT} & \multicolumn{2}{c|}{MMM} & \multicolumn{2}{c|}{HPQ} & \multicolumn{2}{c|}{ADSK} & \multicolumn{2}{c|}{NUE} &  \multicolumn{2}{c|}{PLD} & \multicolumn{2}{c|}{XEL} & \multicolumn{2}{c|}{mean} \\
    %\multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c|}{$\qquad$} \\
    \hline
    & $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$ \\
   
    \hline
QSVM & 0.92 & 0.9 & 0.98 & 0.88 & 0.97 & 0.88 & 0.92 & 0.84 & 0.96 & 0.93 & 0.92 & 0.94 & 0.93 & 0.91 & 0.9 & 0.85 & 0.9 & 0.91 & 0.89 & 0.95 & 0.91 & 0.92 & 0.98 & 0.83 & 0.93  &  0.9 \\
\hline
QNN & 0.76 & 0.75 & 0.83 & 0.72 & 0.78 & 0.75 & 0.75 & 0.75 & 0.79 & 0.76 & 0.74 & 0.78 & 0.82 & 0.78 & 0.77 & 0.72 & 0.78 & 0.77 & 0.73 & 0.72 & 0.77 & 0.78 & 0.82 & 0.65 & 0.78  &  0.74 \\
\hline
SVM & 0.92 & 0.91 & 0.97 & 0.88 & 0.95 & 0.91 & 0.93 & 0.83 & 0.94 & 0.93 & 0.9 & 0.92 & 0.92 & 0.9 & 0.93 & 0.81 & 0.9 & 0.9 & 0.85 & 0.92 & 0.93 & 0.88 & 0.98 & 0.83 & 0.93  &  0.89 \\
\hline
NN & 0.86 & 0.87 & 0.93 & 0.76 & 0.95 & 0.82 & 0.86 & 0.75 & 0.96 & 0.86 & 0.86 & 0.87 & 0.93 & 0.86 & 0.91 & 0.74 & 0.86 & 0.86 & 0.85 & 0.93 & 0.91 & 0.83 & 0.98 & 0.71 & 0.91  &  0.82 \\
\hline
  
\end{tabular}}
\caption{Testing accuracy of 4 ML models for each assets in Case 1. Each score is the average of all 9 time segments.}
\end{subtable}

%\hfill

\begin{subtable}{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ |c|c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| } 
   \hline
    & \multicolumn{2}{c|}{SPYG} & \multicolumn{2}{c|}{SPYV}  & \multicolumn{2}{c|}{VO} & \multicolumn{2}{c|}{VB} & \multicolumn{2}{c|}{QQQ} & \multicolumn{2}{c|}{VEA} & \multicolumn{2}{c|}{VWO} & \multicolumn{2}{c|}{AGG} & \multicolumn{2}{c|}{EMB} & \multicolumn{2}{c|}{JNK} &  \multicolumn{2}{c|}{VNQ} & \multicolumn{2}{c|}{RWX} & \multicolumn{2}{c|}{MBB} & \multicolumn{2}{c|}{MUB} & \multicolumn{2}{c|}{TIP} & \multicolumn{2}{c|}{GLD} &\multicolumn{2}{c|}{mean} \\
    \hline
    & $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$ & $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$\\
   
    \hline
QSVM & 0.97 & 0.87 & 0.93 & 0.92 & 0.93 & 0.88 & 0.91 & 0.91 & 0.96 & 0.86 & 0.93 & 0.92 & 0.9 & 0.87 & 0.96 & 0.93 & 0.92 & 0.84 & 0.96 & 0.92 & 0.92 & 0.92 & 0.91 & 0.92 & 0.96 & 0.9 & 0.95 & 0.9 & 0.93 & 0.93 & 0.89 & 0.91 & 0.93  &  0.9 \\
\hline
QNN & 0.85 & 0.79 & 0.72 & 0.78 & 0.79 & 0.8 & 0.8 & 0.72 & 0.86 & 0.71 & 0.71 & 0.75 & 0.72 & 0.75 & 0.83 & 0.74 & 0.77 & 0.73 & 0.71 & 0.8 & 0.75 & 0.74 & 0.75 & 0.75 & 0.8 & 0.75 & 0.78 & 0.74 & 0.73 & 0.76 & 0.75 & 0.71 & 0.77  &  0.75 \\
\hline
SVM & 0.96 & 0.9 & 0.92 & 0.91 & 0.9 & 0.87 & 0.91 & 0.88 & 0.97 & 0.86 & 0.92 & 0.89 & 0.89 & 0.9 & 0.96 & 0.91 & 0.94 & 0.86 & 0.96 & 0.91 & 0.91 & 0.9 & 0.9 & 0.92 & 0.93 & 0.91 & 0.94 & 0.91 & 0.91 & 0.92 & 0.9 & 0.9 & 0.93  &  0.9 \\
\hline
NN & 0.96 & 0.78 & 0.89 & 0.84 & 0.91 & 0.8 & 0.89 & 0.83 & 0.96 & 0.78 & 0.89 & 0.84 & 0.85 & 0.89 & 0.9 & 0.88 & 0.9 & 0.79 & 0.95 & 0.81 & 0.92 & 0.87 & 0.86 & 0.85 & 0.88 & 0.89 & 0.91 & 0.84 & 0.9 & 0.9 & 0.87 & 0.87 & 0.9  &  0.84 \\
\hline
\end{tabular}}
\caption{Testing accuracy of 4 ML models for each assets in Case 2. Each score is the average of all 9 time segments.}
\end{subtable}

\caption{}
\label{table:qml_scores}
\end{table*}

==> table/vqe_riskadj_return.tex <==
\begin{table}
\begin{subtable}{0.49\textwidth}
\centering
 \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
         Time segment & INDEX & NAIVE & MPT & BL exact & BL VQE & BL QAOA\\
         \hline
0 & 0.445 & 0.378 & 0.368 & 0.439 & 0.437 & 0.347 \\
\hline
1 & 0.214 & 0.186 & 0.163 & 0.207 & 0.207 & 0.221 \\
\hline
2 & -0.069 & -0.015 & 0.037 & 0.052 & 0.065 & 0.023 \\
\hline
3 & 0.164 & 0.184 & 0.102 & 0.105 & 0.162 & 0.136 \\
\hline
4 & 0.251 & 0.238 & 0.232 & 0.241 & 0.237 & 0.305 \\
\hline
5 & -0.044 & -0.034 & -0.154 & -0.041 & 0.007 & -0.036 \\
\hline
6 & 0.17 & 0.223 & 0.3 & 0.207 & 0.18 & 0.144 \\
\hline
7 & -0.318 & -0.392 & -0.394 & -0.372 & -0.373 & -0.46 \\
\hline
8 & 0.147 & 0.227 & 0.273 & 0.166 & 0.166 & 0.092 \\
\hline
mean & 0.107 & 0.111 & 0.103 & 0.112 & 0.121 & 0.086 \\
\hline

    \end{tabular}
}
\caption{CER and SR of back test results of exact solution for case 1 (individual stocks).}
\label{tab:riskadj1}
\end{subtable}


\begin{subtable}{0.5\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
         \hline
         Time segment & \multicolumn{2}{c|}{BL} & \multicolumn{2}{c|}{MPT} & \multicolumn{2}{c|}{NAIVE} & \multicolumn{2}{c|}{INDEX}\\
         \hline
           & CER & SR & CER & SR & CER & SR & CER & SR\\
           \hline
1 & 0.186 & 1.936 & -0.018 & -0.392 & 0.077 & 0.927 & 0.077 & 0.927 \\
\hline
2 & 0.046 & 0.609 & 0.086 & 1.227 & 0.076 & 1.185 & 0.076 & 1.185 \\
\hline
3 & -0.07 & -0.808 & -0.021 & -0.175 & -0.052 & -0.533 & -0.052 & -0.533 \\
\hline
4 & 0.045 & 0.598 & 0.045 & 0.634 & 0.044 & 0.613 & 0.044 & 0.613 \\
\hline
5 & 0.171 & 3.2 & 0.141 & 2.967 & 0.131 & 3.241 & 0.131 & 3.241 \\
\hline
6 & -0.091 & -0.292 & -0.062 & -0.198 & -0.047 & -0.377 & -0.047 & -0.377 \\
\hline
7 & 0.2 & 2.76 & 0.185 & 3.46 & 0.178 & 3.188 & 0.178 & 3.188 \\
\hline
8 & -0.101 & 0.542 & 0.004 & 0.786 & -0.145 & 0.422 & -0.145 & 0.422 \\
\hline
9 & 0.071 & 1.049 & 0.068 & 1.115 & 0.094 & 1.368 & 0.094 & 1.368 \\
\hline
mean &  0.051 & 1.067 & 0.048 & 1.047 & 0.04 & 1.115 & 0.04 & 1.115 \\
         \hline
    \end{tabular}
}
\caption{CER and SR of back test results of exact solution for case 2 (global assets).}
\label{tab:riskadj2}
\end{subtable}


\caption{Risk-adjusted returns.}
\label{tab:riskadj}
\end{table}
